Proust: A Nano Proof Assistant

Proust is a small Racket program offering rudimentary interactive assistance in the development of verified proofs for propositional and predicate logic. It is constructed in stages, some of which are done by students before using it to complete proof exercises, and in parallel with the study of its theoretical underpinnings, including elements of Martin-Lof type theory. The goal is twofold: to demystify some of the machinery behind full-featured proof assistants such as Coq and Agda, and to better integrate the study of formal logic with other core elements of an undergraduate computer science curriculum.

==> eptcsdata.tex <==
\providecommand{\firstpage}{63}
\providecommand{\publicationstatus}{J. Jeuring and J. McCarthy (Eds.): Trends in\\
Functional Programming in Education (TFPIE)\\
EPTCS 230, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.230.5}{10.4204/EPTCS.230.5}}

